UFO: A unified method for controlling Understandability and Faithfulness Objectives in concept-based explanations for CNNs

Concept-based explanations for convolutional neural networks (CNNs) aim to explain model behavior and outputs using a pre-defined set of semantic concepts (e.g., the model recognizes scene class ``bedroom'' based on the presence of concepts ``bed'' and ``pillow''). However, they often do not faithfully (i.e., accurately) characterize the model's behavior and can be too complex for people to understand. Further, little is known about how faithful and understandable different explanation methods are, and how to control these two properties. In this work, we propose UFO, a unified method for controlling Understandability and Faithfulness Objectives in concept-based explanations. UFO formalizes understandability and faithfulness as mathematical objectives and unifies most existing concept-based explanations methods for CNNs. Using UFO, we systematically investigate how explanations change as we turn the knobs of faithfulness and understandability. Our experiments demonstrate a faithfulness-vs-understandability tradeoff: increasing understandability reduces faithfulness. We also provide insights into the ``disagreement problem'' in explainable machine learning, by analyzing when and how concept-based explanations disagree with each other.

==> figures/naps_gini.tex <==
\begin{figure}[t]
    \centering
   \includegraphics[width=\linewidth]{images/naps_gini_big.png}
    \caption{\textbf{Median normalized AP (top) and median gini impurity (bottom) of chosen concepts.} \textcolor{red}{To be updated:} We measure these two quantities for the 16 selected concepts chosen for different settings of faithfulness (sf, lf) and understandability (mu, su, lu). Both quantities generally increase as we increase understandability (i.e., the most understandable explanation selects concepts that are more learnable and correlated to specific scenes).
    % This makes sense as the most understandable explanation is most constrained and will select concepts that are more learnable and correlated to specific scenes.
    }
   % The median normalized AP and median gini impurity value generally increases as we increase the understandability. }
    \label{fig:naps_gini}
\end{figure}

==> figures/remainder.tex <==
\begin{figure*}
    \centering
    \begin{tabular}{c|c|c}
    \toprule
       & \multicolumn{1}{c|}{indoor-transport}  & \multicolumn{1}{c}{indoor-culture } \\
       \midrule
       sf, mu & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder/scene3_0.eps}} & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder/scene5_0.eps} }\\
    sf, su & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder/scene3_1.eps}} & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder/scene5_1.eps}} \\   
       sf, lu & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder/scene3_2.eps}} & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder/scene5_2.eps}} \\\bottomrule
    \end{tabular}
    \caption{\textbf{Visualizing the remainder.}
    For coarse-grained scene classes ``indoor-transport'' and ``indoor-cultural'', we compute  $v = F(x) - h_\text{pred} \circ h_\text{conc}(x)$ and show the top 5 images for which $v_k$ corresponding to those two classes is the largest (i.e., the images that are most poorly explained). 
    By inspection, this suggests that concepts like ``vehicle seats'', ``auditorium seats'', and ``arches'', if labelled in the probe dataset, may help to better explain this model. 
    }
    \label{fig:remainder}
\end{figure*}

==> figures/scene_class_base_rate_vs_explanation_accuracy.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/new_per_class_plots.pdf}
    \caption{\textbf{Scene class base rate vs explanation accuracy}. We consider 3 explanations for the fine-grained scene model using the least faithful (lf) objective and all 3 understandability objectives: lf, mu (most understandable);  lf, su (somewhat understandable); and lf, lu (least understandable).
    % \emph{most understandable} () the least faithful, \emph{most understandable} (lf,mu) explanation, the least faithful, \emph{somewhat understandable} (lf, su) and the least faithful, \emph{least understandable} (lf,lu) explanation.
    We consider the explanation accuracy separately for each scene class and plot each class's base rate versus the difference between two explanations: lf,mu minus lf,lu (\emph{left}) and lf,su minus lf,lu (\emph{right}).  
    We note that while the lf,mu and lf,su explanations are overall less accurate, they are more accurate on the classes with higher base rates. 
    %We measure how increasing understandability of the explanation changes the true positive rate of different classes. Shown are the change in the true positive rate for different fine-grained scene classes for the lf seting. We see that increasing understandability increases the disparity between classes: Classes that have a higher base rate are better explained in the mu setting, whereas classes with lower base rates are better explained in the lu setting.
    }
    \label{fig:tpr_vs_baserate}
\end{figure}

==> rebuttal_cub_no_acc.tex <==
\begin{tabular}{p{1.25cm} l L{3.75cm} L{3.5cm}}
 \toprule
%\multirow{2}{*}{scene} 
%& & Acc & concepts & Acc & concepts & Acc & concepts \\
%\cmidrule(l{3pt}r{3pt}){3-4} \cmidrule(l{3pt}r{3pt}){5-6} \cmidrule(l{3pt}r{3pt}){7-8}
& & somewhat faithful (sf) & less faithful (lf) \\ 
\midrule 
\multirow{6}{*}{\begin{tabular}{c}Great\\ Grey\\ Shrike\end{tabular}} & mu & \textcolor{NavyBlue}{upper-tail-black}, \textcolor{NavyBlue}{main-white}, \textcolor{NavyBlue}{nape-grey} & \textcolor{red}{bill-all-purpose}, \textcolor{red}{tail-striped}, \textcolor{red}{wing-solid} \\
 & su &   \textcolor{red}{wing-spotted}, \textcolor{red}{shape-duck- like}, \textcolor{red}{under-tail-buff} &  \textit{\textcolor{red}{main-yellow}}, \textcolor{red}{crown- blue}, \textcolor{NavyBlue}{bill-size$<$head} \\
& lu &  \textcolor{red}{upper-yellow}, \textcolor{red}{bill- size=head}, \textcolor{red}{bill-seabird} & \textcolor{red}{main-brown}, \textcolor{NavyBlue}{bill-black}, \textit{\textcolor{red}{main-yellow}} \\ \midrule

\multirow{6}{*}{\begin{tabular}{c}Song \\ Sparrow\end{tabular}} & mu & \textit{\textcolor{red}{size-medium}}, \textcolor{NavyBlue}{main-white}, \textcolor{NavyBlue}{breast-black} &  \textit{\textcolor{red}{bill-all-purpose}}, \textcolor{NavyBlue}{tail-striped}, \textit{\textcolor{red}{size-medium}} \\
& su &  \textcolor{NavyBlue}{under-tail-buff}, \textcolor{NavyBlue}{upper- brown}, \textcolor{red}{shape-duck-like} & \textcolor{NavyBlue}{belly-black}, \textcolor{NavyBlue}{belly-white}, \textcolor{red}{forehead-grey} \\
& lu &  \textcolor{red}{upper-yellow}, \textcolor{red}{bill-size =head}, \textit{\textcolor{red}{bill-all-purpose}} &  \textcolor{red}{crown-blue}, \textcolor{red}{main- yellow}, \textcolor{NavyBlue}{breast-striped} \\ \midrule
\multirow{6}{*}{\begin{tabular}{c}Arctic \\Tern \end{tabular}}& mu &  \textcolor{red}{upper-tail-black}, \textcolor{NavyBlue}{wing-pointed}, \textit{\textcolor{NavyBlue}{main-white}} & \textcolor{red}{shape-perching}, \textit{\textcolor{NavyBlue}{upper-yellow}}, \textcolor{red}{bill-buff} \\
& su & \textcolor{red}{wing-spotted}, \textcolor{red}{upper- brown}, \textcolor{red}{shape-duck-like} &  \textit{\textcolor{red}{forehead-white}}, \textcolor{red}{bill-black}, \textcolor{red}{main-brown} \\
& lu & \textit{\textcolor{red}{upper-yellow}}, \textcolor{red}{back- striped}, \textcolor{red}{bill-all-purpose} & \textcolor{red}{crown-blue}, \textit{\textcolor{NavyBlue}{main-white}}, \textit{\textcolor{red}{forehead-white}} \\\bottomrule
\end{tabular}

==> rebuttal_cub_table.tex <==
\begin{tabular}{p{1.25cm} l  c L{3.25cm} c L{3.25cm}}
 \toprule
%\multirow{2}{*}{scene} 
%& & Acc & concepts & Acc & concepts & Acc & concepts \\
%\cmidrule(l{3pt}r{3pt}){3-4} \cmidrule(l{3pt}r{3pt}){5-6} \cmidrule(l{3pt}r{3pt}){7-8}
& & \multicolumn{2}{l}{somewhat faithful (sf)} & \multicolumn{2}{l}{least faithful (lf)} \\ 
\midrule 
Great Grey Shrike & mu & 100.0 & \textcolor{NavyBlue}{upper-tail::black}, \textcolor{NavyBlue}{main::white}, \textcolor{NavyBlue}{nape::grey} & 85.7 & \textcolor{red}{bill::all-purpose}, \textcolor{red}{tail::striped}, \textcolor{red}{wing::solid} \\
& su &  0.0 & \textcolor{red}{wing::spotted}, \textcolor{red}{shape::duck-like}, \textcolor{red}{under-tail::buff} & 100.0 & \textit{\textcolor{red}{main::yellow}}, \textcolor{red}{crown::blue}, \textcolor{NavyBlue}{bill-size::shorter-head} \\
& lu & 0.0 & \textcolor{red}{upper::yellow}, \textcolor{red}{bill-size::same-head}, \textcolor{red}{bill::hooked-seabird} & 57.1 & \textcolor{red}{main::brown}, \textcolor{NavyBlue}{bill::black}, \textit{\textcolor{red}{main::yellow}} \\ \midrule

Song Sparrow & mu & 71.4 & \textit{\textcolor{red}{size::medium}}, \textcolor{NavyBlue}{main::white}, \textcolor{NavyBlue}{breast::black} & 100.0 & \textit{\textcolor{red}{bill::all-purpose}}, \textcolor{NavyBlue}{tail::striped}, \textit{\textcolor{red}{size::medium}} \\
& su &  100.0 & \textcolor{NavyBlue}{under-tail::buff}, \textcolor{NavyBlue}{upper::brown}, \textcolor{red}{shape::duck-like} & 71.4 & \textcolor{NavyBlue}{belly::black}, \textcolor{NavyBlue}{belly::white}, \textcolor{red}{forehead::grey} \\
& lu &  57.1 & \textcolor{red}{upper::yellow}, \textcolor{red}{bill-size::same-head}, \textit{\textcolor{red}{bill::all-purpose}} & 28.6 & \textcolor{red}{crown::blue}, \textcolor{red}{main::yellow}, \textcolor{NavyBlue}{breast::striped} \\ \midrule
Artic Tern & mu & 100.0 & \textcolor{red}{upper-tail::black}, \textcolor{NavyBlue}{wing::pointed
}, \textit{\textcolor{NavyBlue}{main::white}} & 81.8 & \textcolor{red}{shape::perching}, \textit{\textcolor{NavyBlue}{upper::yellow}}, \textcolor{red}{bill::buff} \\
& su & 90.9 & \textcolor{red}{wing::spotted}, \textcolor{red}{upper::brown}, \textcolor{red}{shape::duck-like} & 81.8 & \textit{\textcolor{red}{forehead::white}}, \textcolor{red}{bill::black}, \textcolor{red}{main::brown} \\
& lu & 72.7 & \textit{\textcolor{red}{upper::yellow}}, \textcolor{red}{back::striped}, \textcolor{red}{bill::all-purpose} & 72.7 & \textcolor{red}{crown::blue}, \textit{\textcolor{NavyBlue}{main::white}}, \textit{\textcolor{red}{forehead::white}} \\\bottomrule
%Least-Tern & lf & 90.0 & \textcolor{NavyBlue}{forehead::white}, \textcolor{NavyBlue}{wing::solid}, \textcolor{red}{crown::white} & 90.0 & \textcolor{red}{forehead::white}, \textcolor{red}{belly::black}, \textcolor{NavyBlue}{forehead::grey} & 40.0 & \textcolor{red}{belly::black}, \textcolor{red}{crown::blue}, \textcolor{red}{bill::hooked-seabird} \\
%Nashville-Warbler & lf & 100.0 & \textcolor{NavyBlue}{back::yellow}, \textcolor{NavyBlue}{upper::yellow}, \textcolor{NavyBlue}{bill-size::shorter-head} & 100.0 & \textcolor{NavyBlue}{main::buff}, \textcolor{red}{forehead::white}, \textcolor{red}{shape::perching-like} & 50.0 & \textcolor{NavyBlue}{main::yellow}, \textcolor{red}{crown::blue}, \textcolor{red}{upper::buff} \\
\end{tabular}

==> remainder_all.tex <==
\begin{figure*}[t]
    \centering
    \begin{tabular}{c|c|c}
    \toprule
 & attic (sloped roof?) & bedchamber (bed curtains?) \\\midrule
sf, mu & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene0_0.pdf}} & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene2_0.pdf}} \\ 
sf, su & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene0_1.pdf}} & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene2_1.pdf}} \\ 
sf, lu & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene0_2.pdf}} & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene2_2.pdf}} \\ 
\midrule
& conference-room (large table?) & dining-room (table with chairs?) \\\midrule
sf, mu & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene4_0.pdf}} & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene6_0.pdf}} \\ 
sf, su & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene4_1.pdf}} & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene6_1.pdf}} \\ 
sf, lu & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene4_2.pdf}} & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene6_2.pdf}} \\ 
\midrule
& waiting-room (multiple chairs?) & television-room (black rectangle?) \\\midrule
sf, mu & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene18_0.pdf}} & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene17_0.pdf}} \\ 
sf, su & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene18_1.pdf}} & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene17_1.pdf}} \\ 
sf, lu & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene18_2.pdf}} & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene17_2.pdf}} \\ 
\midrule
& recreation-room (pool table?) & residential-neighborhood (road with building?) \\\midrule
sf, mu & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene13_0.pdf}} & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene14_0.pdf}} \\ 
sf, su & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene13_1.pdf}} & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene14_1.pdf}} \\ 
sf, lu & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene13_2.pdf}} & \raisebox{-0.4\totalheight}{\includegraphics[width=0.4\textwidth]{images/remainder_all/scene14_2.pdf}} \\ 
 \bottomrule 
\end{tabular}
\caption{\textbf{Visualizing the remainder}. We compute  $v = F(x) - h_\text{pred} \circ h_\text{conc}(x)$ and show the top 5 images for which $v_k$ corresponding to these classes is the largest (i.e., the images that are most poorly explained). We show images from classes that appear to have a pattern, for example, for ``bedchamber'', we see that beds with bed-curtains appear to be important to the prediction, similarly for ``attic'', we see that it's the presence of a sloping roof. We propose additional concepts for each class in parenthesis. }
\label{fig:remainder_all}
\end{figure*}

==> tables/finegrained_attr.tex <==
\begin{tabular}{p{2cm} l  c L{3.5cm} c L{3.5cm} c L{3.5cm}}
 \toprule
%\multirow{2}{*}{scene} 
%& & Acc & concepts & Acc & concepts & Acc & concepts \\
%\cmidrule(l{3pt}r{3pt}){3-4} \cmidrule(l{3pt}r{3pt}){5-6} \cmidrule(l{3pt}r{3pt}){7-8}
& & \multicolumn{2}{l}{most understandable (mu)} & \multicolumn{2}{l}{somewhat understandable (su)} & \multicolumn{2}{l}{least understandable (lu)} \\ 
\midrule 

%\multicolumn{7}{l}{\textbf{somewhat faithful (sf)}}\\
%\toprule
%\multirow{2}{*}{fine-grained scene} & & \multicolumn{2}{c|}{most understandable (mu)} & \multicolumn{2}{c|}{somewhat understandable (su)} & \multicolumn{2}{c}{least understandable (lu)} \\ \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}
%& & Acc & concepts & Acc & concepts & Acc & concepts \\ \midrule 

%attic & sf & 0.0 & \textcolor{red}{baby buggy}, \textcolor{red}{central reservation}, \textcolor{NavyBlue}{pillow} & 0.0 & \textcolor{red}{cross}, \textcolor{red}{newspaper}, \textcolor{red}{apparel} & 0.0 & \textcolor{NavyBlue}{lamp}, \textcolor{red}{table}, \textcolor{red}{painting} \\ 
bathroom & sf& 60.5 & \textcolor{red}{baby buggy}, \textcolor{NavyBlue}{sink}, \textcolor{NavyBlue}{\emph{countertop}} & 18.5 & \textcolor{NavyBlue}{wardrobe}, \textcolor{NavyBlue}{soap dispenser}, \textcolor{NavyBlue}{curtain} & 99.2 & \textcolor{NavyBlue}{\emph{countertop}}, \textcolor{red}{\emph{table}}, \textcolor{red}{mountain} \\ 
 &lf  & 96.8 & \textcolor{red}{work surface}, \textcolor{red}{\emph{bed}}, \textcolor{red}{television} & 99.2 & \textcolor{red}{sofa}, \textcolor{red}{\emph{table}}, \textcolor{red}{\emph{bed}} & 91.1 & \textcolor{NavyBlue}{cabinet}, \textcolor{red}{ceiling}, \textcolor{NavyBlue}{door} \\ 
 \midrule
%bedchamber & sf & 0.0 & \textcolor{red}{central reservation}, \textcolor{red}{baby buggy}, \textcolor{NavyBlue}{pillow} & 0.0 & \textcolor{red}{cross}, \textcolor{NavyBlue}{bed}, \textcolor{red}{soap dispenser} & 8.8 & \textcolor{NavyBlue}{lamp}, \textcolor{red}{refrigerator}, \textcolor{NavyBlue}{countertop} \\ 
bedroom  & sf& 61.7 & \textcolor{NavyBlue}{\emph{pillow}}, \textcolor{red}{baby buggy}, \textcolor{red}{central reservation} & 91.4 & \textcolor{red}{cross}, \textcolor{NavyBlue}{bed}, \textcolor{NavyBlue}{\emph{pillow}} & 85.9 & \textcolor{NavyBlue}{lamp}, \textcolor{red}{refrigerator}, \textcolor{NavyBlue}{countertop} \\
 &lf& 83.6 & \textcolor{red}{\emph{sink}}, \textcolor{red}{pool table}, \textcolor{red}{skyscraper} & 99.2 & \textcolor{red}{\emph{sink}}, \textcolor{red}{work surface}, \textcolor{red}{building} & 78.1 & \textcolor{NavyBlue}{curtain}, \textcolor{NavyBlue}{windowpane}, \textcolor{red}{chair} \\ 
 \midrule
%conference-room & sf & 0.0 & \textcolor{red}{baby buggy}, \textcolor{NavyBlue}{floor}, \textcolor{red}{pillow} & 0.0 & \textcolor{red}{newspaper}, \textcolor{red}{cross}, \textcolor{NavyBlue}{table} & 40.9 & \textcolor{red}{countertop}, \textcolor{red}{lamp}, \textcolor{NavyBlue}{table} \\ 
crosswalk & sf & 0.0 & \textcolor{NavyBlue}{baby buggy}, \textcolor{NavyBlue}{central reservation}, \textcolor{red}{floor} & 0.0 & \textcolor{NavyBlue}{cross}, \textcolor{NavyBlue}{newspaper}, \textcolor{NavyBlue}{step} & 0.0 & \textcolor{NavyBlue}{car}, \textcolor{red}{mountain}, \textcolor{NavyBlue}{\emph{truck}} \\ 
 &lf& 0.0 & \textcolor{red}{skyscraper}, \textcolor{red}{\emph{work surface}}, \textcolor{red}{\emph{sink}} & 0.0 & \textcolor{red}{\emph{sink}}, \textcolor{red}{chair}, \textcolor{red}{\emph{work surface}} & 2.2 & \textcolor{NavyBlue}{\emph{truck}}, \textcolor{red}{door}, \textcolor{red}{cabinet} \\ 
 \midrule
%dining-room & sf & 18.0 & \textcolor{red}{baby buggy}, \textcolor{red}{central reservation}, \textcolor{NavyBlue}{floor} & 75.0 & \textcolor{NavyBlue}{table}, \textcolor{NavyBlue}{windowpane}, \textcolor{NavyBlue}{ceiling} & 82.0 & \textcolor{NavyBlue}{refrigerator}, \textcolor{NavyBlue}{table}, \textcolor{red}{lamp} \\ 
downtown & sf & 11.1 & \textcolor{NavyBlue}{baby buggy}, \textcolor{red}{\emph{floor}}, \textcolor{NavyBlue}{central reservation} & 4.4 & \textcolor{NavyBlue}{step}, \textcolor{NavyBlue}{newspaper}, \textcolor{NavyBlue}{cross} & 53.3 & \textcolor{NavyBlue}{building}, \textcolor{red}{\emph{floor}}, \textcolor{red}{tree} \\ 
 &lf& 4.4 & \textcolor{red}{\emph{sink}}, \textcolor{red}{bed}, \textcolor{red}{ceiling} & 0.0 & \textcolor{red}{\emph{ceiling}}, \textcolor{red}{cabinet}, \textcolor{red}{\emph{sink}} & 0.0 & \textcolor{red}{wall}, \textcolor{red}{\emph{floor}}, \textcolor{red}{\emph{ceiling}} \\ 
 \midrule
%highway & sf & 85.7 & \textcolor{NavyBlue}{central reservation}, \textcolor{red}{floor}, \textcolor{red}{wall} & 97.1 & \textcolor{NavyBlue}{step}, \textcolor{NavyBlue}{newspaper}, \textcolor{NavyBlue}{apparel} & 94.3 & \textcolor{NavyBlue}{mountain}, \textcolor{NavyBlue}{car}, \textcolor{red}{building} \\ 
%hotel-room & sf & 15.1 & \textcolor{red}{central reservation}, \textcolor{NavyBlue}{pillow}, \textcolor{red}{baby buggy} & 0.0 & \textcolor{red}{cross}, \textcolor{NavyBlue}{bed}, \textcolor{NavyBlue}{pillow} & 11.3 & \textcolor{NavyBlue}{lamp}, \textcolor{red}{refrigerator}, \textcolor{NavyBlue}{countertop} \\ 
kitchen & sf & 58.2 & \textcolor{NavyBlue}{sink}, \textcolor{NavyBlue}{bowl}, \textcolor{NavyBlue}{faucet} & 11.0 & \textcolor{NavyBlue}{soap dispenser}, \textcolor{NavyBlue}{wardrobe}, \textcolor{NavyBlue}{windowpane} & 89.0 & \textcolor{NavyBlue}{refrigerator}, \textcolor{red}{mountain}, \textcolor{red}{camera} \\ 
 &lf& 82.4 & \textcolor{red}{\emph{bed}}, \textcolor{red}{pool table}, \textcolor{NavyBlue}{\emph{work surface}} & 92.3 & \textcolor{NavyBlue}{\emph{work surface}}, \textcolor{red}{\emph{bed}}, \textcolor{red}{sofa} & 91.2 & \textcolor{NavyBlue}{cabinet}, \textcolor{NavyBlue}{wall socket}, \textcolor{red}{curtain} \\
\midrule
%living-room & sf & 57.1 & \textcolor{red}{central reservation}, \textcolor{red}{baby buggy}, \textcolor{NavyBlue}{sofa} & 12.9 & \textcolor{red}{cross}, \textcolor{NavyBlue}{book}, \textcolor{NavyBlue}{ceiling} & 21.4 & \textcolor{NavyBlue}{painting}, \textcolor{red}{keyboard}, \textcolor{NavyBlue}{lamp} \\ 
parking-garage & sf & 0.0 & \textcolor{NavyBlue}{baby buggy}, \textcolor{red}{\emph{floor}}, \textcolor{NavyBlue}{central reservation} & 0.0 & \textcolor{NavyBlue}{newspaper}, \textcolor{NavyBlue}{cross}, \textcolor{NavyBlue}{apparel} & 0.0 & \textcolor{NavyBlue}{building}, \textcolor{NavyBlue}{lamp}, \textcolor{red}{mountain} \\ 
 (outdoor) &lf& 0.0 & \textcolor{red}{skyscraper}, \textcolor{red}{bed}, \textcolor{red}{\emph{ceiling}} & 0.0 & \textcolor{red}{sink}, \textcolor{red}{vase}, \textcolor{red}{\emph{ceiling}} & 2.3 & \textcolor{NavyBlue}{door}, \textcolor{red}{\emph{floor}}, \textcolor{NavyBlue}{truck} \\  \midrule
%recreation-room & sf & 33.9 & \textcolor{red}{baby buggy}, \textcolor{NavyBlue}{ceiling}, \textcolor{NavyBlue}{floor} & 78.6 & \textcolor{red}{cross}, \textcolor{red}{newspaper}, \textcolor{NavyBlue}{ceiling} & 42.9 & \textcolor{NavyBlue}{painting}, \textcolor{NavyBlue}{floor}, \textcolor{red}{cross} \\ 
%residential-neighborhood  & sf& 61.4 & \textcolor{red}{floor}, \textcolor{NavyBlue}{central reservation}, \textcolor{NavyBlue}{plant} & 0.0 & \textcolor{NavyBlue}{step}, \textcolor{NavyBlue}{newspaper}, \textcolor{NavyBlue}{apparel} & 49.1 & \textcolor{NavyBlue}{tree}, \textcolor{NavyBlue}{car}, \textcolor{NavyBlue}{building} \\ 
%skyscraper & sf & 0.0 & \textcolor{red}{floor}, \textcolor{NavyBlue}{baby buggy}, \textcolor{red}{wall} & 2.7 & \textcolor{NavyBlue}{newspaper}, \textcolor{NavyBlue}{step}, \textcolor{NavyBlue}{soap dispenser} & 94.6 & \textcolor{NavyBlue}{building}, \textcolor{NavyBlue}{camera}, \textcolor{red}{car} \\ 
street & sf & 0.0 & \textcolor{NavyBlue}{baby buggy}, \textcolor{red}{\emph{floor}}, \textcolor{NavyBlue}{central reservation} & 0.0 & \textcolor{NavyBlue}{cross}, \textcolor{NavyBlue}{newspaper}, \textcolor{NavyBlue}{step} & 90.8 & \textcolor{NavyBlue}{car}, \textcolor{NavyBlue}{building}, \textcolor{red}{\emph{floor}} \\ 
 &lf& 78.2 & \textcolor{red}{skyscraper}, \textcolor{red}{\emph{sink}}, \textcolor{red}{work surface} & 100.0 & \textcolor{red}{\emph{sink}}, \textcolor{red}{cabinet}, \textcolor{red}{sofa} & 97.7 & \textcolor{NavyBlue}{truck}, \textcolor{red}{wall}, \textcolor{red}{curtain} \\ 
\iffalse
 \midrule
television-room & sf & 38.9 & \textcolor{red}{baby buggy}, \textcolor{red}{central reservation}, \textcolor{NavyBlue}{\emph{painting}} & 81.9 & \textcolor{red}{\emph{cross}}, \textcolor{NavyBlue}{book}, \textcolor{red}{newspaper} & 70.8 & \textcolor{NavyBlue}{lamp}, \textcolor{NavyBlue}{\emph{painting}}, \textcolor{red}{\emph{cross}} \\ 
 &lf& 29.2 & \textcolor{red}{pool table}, \textcolor{red}{\emph{sink}}, \textcolor{red}{skyscraper} & 9.7 & \textcolor{red}{\emph{sink}}, \textcolor{red}{work surface}, \textcolor{red}{tree} & 41.7 & \textcolor{NavyBlue}{cabinet}, \textcolor{NavyBlue}{curtain}, \textcolor{NavyBlue}{chair} \\ 
\midrule
waiting-room & sf & 0.0 & \textcolor{NavyBlue}{sofa}, \textcolor{red}{baby buggy}, \textcolor{NavyBlue}{\emph{floor}} & 0.0 & \textcolor{red}{cross}, \textcolor{red}{soap dispenser}, \textcolor{red}{newspaper} & 4.8 & \textcolor{NavyBlue}{painting}, \textcolor{red}{lamp}, \textcolor{NavyBlue}{table} \\ 
 &lf& 0.0 & \textcolor{red}{\emph{bed}}, \textcolor{red}{pool table}, \textcolor{red}{\emph{work surface}} & 0.0 & \textcolor{red}{\emph{work surface}}, \textcolor{red}{sink}, \textcolor{red}{\emph{bed}} & 38.1 & \textcolor{NavyBlue}{chair}, \textcolor{NavyBlue}{\emph{floor}}, \textcolor{red}{cabinet} \\
\fi
%youth-hostel & 15.9 & \textcolor{NavyBlue}{pillow}, \textcolor{red}{central reservation}, \textcolor{red}{baby buggy} & 0.0 & \textcolor{NavyBlue}{bed}, \textcolor{red}{cross}, \textcolor{NavyBlue}{pillow} & 0.0 & \textcolor{NavyBlue}{lamp}, \textcolor{red}{refrigerator}, \textcolor{NavyBlue}{countertop} \\ 
\bottomrule
\end{tabular}

==> tables/finegrained_attr_v1.tex <==
\begin{tabular}{l |c L{3.5cm}| c L{3.5cm}| c L{3.5cm}}
 \toprule
\multicolumn{7}{l}{\textbf{somewhat faithful (sf)}}\\
\toprule
\multirow{2}{*}{fine-grain scene} & \multicolumn{2}{c|}{most understandable (mu)} & \multicolumn{2}{c|}{somewhat understandable (su)} & \multicolumn{2}{c}{least understandable (lu)} \\ \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}
& Acc & concepts & Acc & concepts & Acc & concepts \\ \midrule 
%attic & 0.0 & \textcolor{red}{baby buggy}, \textcolor{red}{central reservation}, \textcolor{NavyBlue}{pillow} & 0.0 & \textcolor{red}{cross}, \textcolor{red}{newspaper}, \textcolor{red}{apparel} & 0.0 & \textcolor{NavyBlue}{lamp}, \textcolor{red}{table}, \textcolor{red}{painting} \\ 
bathroom & 60.5 & \textcolor{red}{baby buggy}, \textcolor{NavyBlue}{sink}, \textcolor{NavyBlue}{\emph{countertop}} & 18.5 & \textcolor{NavyBlue}{wardrobe}, \textcolor{NavyBlue}{soap dispenser}, \textcolor{NavyBlue}{curtain} & 99.2 & \textcolor{NavyBlue}{\emph{countertop}}, \textcolor{red}{\emph{table}}, \textcolor{red}{mountain} \\ 
%bedchamber & 0.0 & \textcolor{red}{central reservation}, \textcolor{red}{baby buggy}, \textcolor{NavyBlue}{pillow} & 0.0 & \textcolor{red}{cross}, \textcolor{NavyBlue}{bed}, \textcolor{red}{soap dispenser} & 8.8 & \textcolor{NavyBlue}{lamp}, \textcolor{red}{refrigerator}, \textcolor{NavyBlue}{countertop} \\ 
bedroom & 61.7 & \textcolor{NavyBlue}{\emph{pillow}}, \textcolor{red}{baby buggy}, \textcolor{red}{central reservation} & 91.4 & \textcolor{red}{cross}, \textcolor{NavyBlue}{bed}, \textcolor{NavyBlue}{\emph{pillow}} & 85.9 & \textcolor{NavyBlue}{lamp}, \textcolor{red}{refrigerator}, \textcolor{NavyBlue}{countertop} \\ 
%conference-room & 0.0 & \textcolor{red}{baby buggy}, \textcolor{NavyBlue}{floor}, \textcolor{red}{pillow} & 0.0 & \textcolor{red}{newspaper}, \textcolor{red}{cross}, \textcolor{NavyBlue}{table} & 40.9 & \textcolor{red}{countertop}, \textcolor{red}{lamp}, \textcolor{NavyBlue}{table} \\ 
crosswalk & 0.0 & \textcolor{NavyBlue}{baby buggy}, \textcolor{NavyBlue}{central reservation}, \textcolor{red}{floor} & 0.0 & \textcolor{NavyBlue}{cross}, \textcolor{NavyBlue}{newspaper}, \textcolor{NavyBlue}{step} & 0.0 & \textcolor{NavyBlue}{car}, \textcolor{red}{mountain}, \textcolor{NavyBlue}{truck} \\ 
%dining-room & 18.0 & \textcolor{red}{baby buggy}, \textcolor{red}{central reservation}, \textcolor{NavyBlue}{floor} & 75.0 & \textcolor{NavyBlue}{table}, \textcolor{NavyBlue}{windowpane}, \textcolor{NavyBlue}{ceiling} & 82.0 & \textcolor{NavyBlue}{refrigerator}, \textcolor{NavyBlue}{table}, \textcolor{red}{lamp} \\ 
downtown & 11.1 & \textcolor{NavyBlue}{baby buggy}, \textcolor{red}{floor}, \textcolor{NavyBlue}{central reservation} & 4.4 & \textcolor{NavyBlue}{step}, \textcolor{NavyBlue}{newspaper}, \textcolor{NavyBlue}{cross} & 53.3 & \textcolor{NavyBlue}{building}, \textcolor{red}{floor}, \textcolor{red}{tree} \\ 
%highway & 85.7 & \textcolor{NavyBlue}{central reservation}, \textcolor{red}{floor}, \textcolor{red}{wall} & 97.1 & \textcolor{NavyBlue}{step}, \textcolor{NavyBlue}{newspaper}, \textcolor{NavyBlue}{apparel} & 94.3 & \textcolor{NavyBlue}{mountain}, \textcolor{NavyBlue}{car}, \textcolor{red}{building} \\ 
%hotel-room & 15.1 & \textcolor{red}{central reservation}, \textcolor{NavyBlue}{pillow}, \textcolor{red}{baby buggy} & 0.0 & \textcolor{red}{cross}, \textcolor{NavyBlue}{bed}, \textcolor{NavyBlue}{pillow} & 11.3 & \textcolor{NavyBlue}{lamp}, \textcolor{red}{refrigerator}, \textcolor{NavyBlue}{countertop} \\ 
kitchen & 58.2 & \textcolor{NavyBlue}{sink}, \textcolor{NavyBlue}{bowl}, \textcolor{NavyBlue}{faucet} & 11.0 & \textcolor{NavyBlue}{soap dispenser}, \textcolor{NavyBlue}{wardrobe}, \textcolor{NavyBlue}{windowpane} & 89.0 & \textcolor{NavyBlue}{refrigerator}, \textcolor{red}{mountain}, \textcolor{red}{camera} \\ 
%living-room & 57.1 & \textcolor{red}{central reservation}, \textcolor{red}{baby buggy}, \textcolor{NavyBlue}{sofa} & 12.9 & \textcolor{red}{cross}, \textcolor{NavyBlue}{book}, \textcolor{NavyBlue}{ceiling} & 21.4 & \textcolor{NavyBlue}{painting}, \textcolor{red}{keyboard}, \textcolor{NavyBlue}{lamp} \\ 
parking-garage/outdoor & 0.0 & \textcolor{NavyBlue}{baby buggy}, \textcolor{red}{floor}, \textcolor{NavyBlue}{central reservation} & 0.0 & \textcolor{NavyBlue}{newspaper}, \textcolor{NavyBlue}{cross}, \textcolor{NavyBlue}{apparel} & 0.0 & \textcolor{NavyBlue}{building}, \textcolor{NavyBlue}{lamp}, \textcolor{red}{mountain} \\ 
%recreation-room & 33.9 & \textcolor{red}{baby buggy}, \textcolor{NavyBlue}{ceiling}, \textcolor{NavyBlue}{floor} & 78.6 & \textcolor{red}{cross}, \textcolor{red}{newspaper}, \textcolor{NavyBlue}{ceiling} & 42.9 & \textcolor{NavyBlue}{painting}, \textcolor{NavyBlue}{floor}, \textcolor{red}{cross} \\ 
%residential-neighborhood & 61.4 & \textcolor{red}{floor}, \textcolor{NavyBlue}{central reservation}, \textcolor{NavyBlue}{plant} & 0.0 & \textcolor{NavyBlue}{step}, \textcolor{NavyBlue}{newspaper}, \textcolor{NavyBlue}{apparel} & 49.1 & \textcolor{NavyBlue}{tree}, \textcolor{NavyBlue}{car}, \textcolor{NavyBlue}{building} \\ 
%skyscraper & 0.0 & \textcolor{red}{floor}, \textcolor{NavyBlue}{baby buggy}, \textcolor{red}{wall} & 2.7 & \textcolor{NavyBlue}{newspaper}, \textcolor{NavyBlue}{step}, \textcolor{NavyBlue}{soap dispenser} & 94.6 & \textcolor{NavyBlue}{building}, \textcolor{NavyBlue}{camera}, \textcolor{red}{car} \\ 
street & 0.0 & \textcolor{NavyBlue}{baby buggy}, \textcolor{red}{floor}, \textcolor{NavyBlue}{central reservation} & 0.0 & \textcolor{NavyBlue}{cross}, \textcolor{NavyBlue}{newspaper}, \textcolor{NavyBlue}{step} & 90.8 & \textcolor{NavyBlue}{car}, \textcolor{NavyBlue}{building}, \textcolor{red}{floor} \\ 
television-room & 38.9 & \textcolor{red}{baby buggy}, \textcolor{red}{central reservation}, \textcolor{NavyBlue}{painting} & 81.9 & \textcolor{red}{cross}, \textcolor{NavyBlue}{book}, \textcolor{red}{newspaper} & 70.8 & \textcolor{NavyBlue}{lamp}, \textcolor{NavyBlue}{painting}, \textcolor{red}{cross} \\ 
waiting-room & 0.0 & \textcolor{NavyBlue}{sofa}, \textcolor{red}{baby buggy}, \textcolor{NavyBlue}{floor} & 0.0 & \textcolor{red}{cross}, \textcolor{red}{soap dispenser}, \textcolor{red}{newspaper} & 4.8 & \textcolor{NavyBlue}{painting}, \textcolor{red}{lamp}, \textcolor{NavyBlue}{table} \\ 
%youth-hostel & 15.9 & \textcolor{NavyBlue}{pillow}, \textcolor{red}{central reservation}, \textcolor{red}{baby buggy} & 0.0 & \textcolor{NavyBlue}{bed}, \textcolor{red}{cross}, \textcolor{NavyBlue}{pillow} & 0.0 & \textcolor{NavyBlue}{lamp}, \textcolor{red}{refrigerator}, \textcolor{NavyBlue}{countertop} \\ 
 \toprule
\multicolumn{7}{l}{\textbf{least faithful (lf)}}\\
\toprule
\multirow{2}{*}{fine-grain scene} & \multicolumn{2}{c|}{most understandable (mu)} & \multicolumn{2}{c|}{somewhat understandable (su)} & \multicolumn{2}{c}{least understandable (lu)} \\ \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}
& Acc & concepts & Acc & concepts & Acc & concepts \\ \midrule 
bathroom & 96.8 & \textcolor{red}{work surface}, \textcolor{red}{\emph{bed}}, \textcolor{red}{television} & 99.2 & \textcolor{red}{sofa}, \textcolor{red}{\emph{table}}, \textcolor{red}{\emph{bed}} & 91.1 & \textcolor{NavyBlue}{cabinet}, \textcolor{red}{ceiling}, \textcolor{NavyBlue}{door} \\ 
bedroom & 83.6 & \textcolor{red}{sink}, \textcolor{red}{pool table}, \textcolor{red}{skyscraper} & 99.2 & \textcolor{red}{sink}, \textcolor{red}{work surface}, \textcolor{red}{building} & 78.1 & \textcolor{NavyBlue}{curtain}, \textcolor{NavyBlue}{windowpane}, \textcolor{red}{chair} \\ 
crosswalk & 0.0 & \textcolor{red}{skyscraper}, \textcolor{red}{work surface}, \textcolor{red}{sink} & 0.0 & \textcolor{red}{sink}, \textcolor{red}{chair}, \textcolor{red}{work surface} & 2.2 & \textcolor{NavyBlue}{truck}, \textcolor{red}{door}, \textcolor{red}{cabinet} \\ 
downtown & 4.4 & \textcolor{red}{sink}, \textcolor{red}{bed}, \textcolor{red}{ceiling} & 0.0 & \textcolor{red}{ceiling}, \textcolor{red}{cabinet}, \textcolor{red}{sink} & 0.0 & \textcolor{red}{wall}, \textcolor{red}{floor}, \textcolor{red}{ceiling} \\ 
kitchen & 82.4 & \textcolor{red}{bed}, \textcolor{red}{pool table}, \textcolor{NavyBlue}{work surface} & 92.3 & \textcolor{NavyBlue}{work surface}, \textcolor{red}{bed}, \textcolor{red}{sofa} & 91.2 & \textcolor{NavyBlue}{cabinet}, \textcolor{NavyBlue}{wall socket}, \textcolor{red}{curtain} \\ 
parking-garage/outdoor & 0.0 & \textcolor{red}{skyscraper}, \textcolor{red}{bed}, \textcolor{red}{ceiling} & 0.0 & \textcolor{red}{sink}, \textcolor{red}{vase}, \textcolor{red}{ceiling} & 2.3 & \textcolor{NavyBlue}{door}, \textcolor{red}{floor}, \textcolor{NavyBlue}{truck} \\ 
street & 78.2 & \textcolor{red}{skyscraper}, \textcolor{red}{sink}, \textcolor{red}{work surface} & 100.0 & \textcolor{red}{sink}, \textcolor{red}{cabinet}, \textcolor{red}{sofa} & 97.7 & \textcolor{NavyBlue}{truck}, \textcolor{red}{wall}, \textcolor{red}{curtain} \\ 
television-room & 29.2 & \textcolor{red}{pool table}, \textcolor{red}{sink}, \textcolor{red}{skyscraper} & 9.7 & \textcolor{red}{sink}, \textcolor{red}{work surface}, \textcolor{red}{tree} & 41.7 & \textcolor{NavyBlue}{cabinet}, \textcolor{NavyBlue}{curtain}, \textcolor{NavyBlue}{chair} \\ 
waiting-room & 0.0 & \textcolor{red}{bed}, \textcolor{red}{pool table}, \textcolor{red}{work surface} & 0.0 & \textcolor{red}{work surface}, \textcolor{red}{sink}, \textcolor{red}{bed} & 38.1 & \textcolor{NavyBlue}{chair}, \textcolor{NavyBlue}{floor}, \textcolor{red}{cabinet} \\ \bottomrule
\end{tabular}

==> tables/grouped_attr_v1.tex <==
\begin{tabular}{l |c L{3.5cm}| c L{3.5cm}| c L{3.5cm}}
 \toprule
\multicolumn{7}{l}{\textbf{somewhat faithful}}\\
\toprule
\multirow{2}{*}{scene group} & \multicolumn{2}{c|}{most understandable} & \multicolumn{2}{c|}{somewhat understandable} & \multicolumn{2}{c}{least understandable} \\ \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}
& TPR & concepts & TPR & concepts & TPR & concepts \\ \midrule 
%cabins, gardens, farms& 0.0 & \textcolor{NavyBlue}{tree}, \textcolor{red}{vending machine}, \textcolor{red}{bridge} & 17.6 & \textcolor{red}{brush}, \textcolor{red}{towel}, \textcolor{NavyBlue}{tree} & 29.8 & \textcolor{NavyBlue}{earth}, \textcolor{red}{spotlight}, \textcolor{red}{sky} \\ 
comm-buildings& 71.9 & \textcolor{NavyBlue}{building}, \textcolor{NavyBlue}{road}, \textcolor{red}{bridge} & 76.0 & \textcolor{NavyBlue}{building}, \textcolor{NavyBlue}{van}, \textcolor{NavyBlue}{plate} & 72.5 & \textcolor{NavyBlue}{building}, \textcolor{red}{fence}, \textcolor{NavyBlue}{backpack} \\
cultural-historic& 47.0 & \textcolor{NavyBlue}{building}, \textcolor{red}{bridge}, \textcolor{red}{floor} & 50.9 & \textcolor{red}{towel}, \textcolor{red}{fluorescent}, \textcolor{NavyBlue}{sconce} & 59.9 & \textcolor{red}{fence}, \textcolor{NavyBlue}{building}, \textcolor{NavyBlue}{spotlight} \\ 
%forest, field, jungle& 65.6 & \textcolor{NavyBlue}{tree}, \textcolor{red}{building}, \textcolor{red}{road} & 80.9 & \textcolor{NavyBlue}{tree}, \textcolor{red}{plate}, \textcolor{red}{building} & 65.6 & \textcolor{red}{floor}, \textcolor{red}{mountain}, \textcolor{red}{building} \\ 
home-hotel& 71.2 & \textcolor{NavyBlue}{floor}, \textcolor{NavyBlue}{wall}, \textcolor{NavyBlue}{wall socket} & 91.9 & \textcolor{red}{fluorescent}, \textcolor{NavyBlue}{towel}, \textcolor{red}{brush} & 92.9 & \textcolor{NavyBlue}{beam}, \textcolor{red}{backpack}, \textcolor{red}{mountain} \\ 
indoor-culture & 0.0 & \textcolor{red}{sky}, \textcolor{red}{tree}, \textcolor{NavyBlue}{floor} & 1.4 & \textcolor{red}{towel}, \textcolor{NavyBlue}{brush}, \textcolor{NavyBlue}{fluorescent} & 25.5 & \textcolor{NavyBlue}{spotlight}, \textcolor{red}{toilet tissue}, \textcolor{red}{oven} \\ 
%indoor-sports & 0.0 & \textcolor{red}{sky}, \textcolor{NavyBlue}{floor}, \textcolor{NavyBlue}{vending machine} & 0.0 & \textcolor{NavyBlue}{towel}, \textcolor{red}{fluorescent}, \textcolor{red}{plate} & 16.4 & \textcolor{NavyBlue}{fence}, \textcolor{red}{backpack}, \textcolor{NavyBlue}{toilet tissue} \\ 
%indoor-transport& 0.0 & \textcolor{NavyBlue}{floor}, \textcolor{red}{tree}, \textcolor{NavyBlue}{road} & 0.0 & \textcolor{red}{brush}, \textcolor{red}{plate}, \textcolor{red}{towel} & 6.8 & \textcolor{red}{earth}, \textcolor{NavyBlue}{floor}, \textcolor{NavyBlue}{beam} \\ 
%industrial/construction& 0.0 & \textcolor{NavyBlue}{building}, \textcolor{NavyBlue}{sky}, \textcolor{red}{floor} & 0.0 & \textcolor{red}{brush}, \textcolor{NavyBlue}{van}, \textcolor{red}{tree} & 0.0 & \textcolor{red}{backpack}, \textcolor{red}{floor}, \textcolor{NavyBlue}{car} \\ 
%man-made elements& 7.7 & \textcolor{NavyBlue}{bridge}, \textcolor{NavyBlue}{sky}, \textcolor{red}{floor} & 0.0 & \textcolor{NavyBlue}{fluorescent}, \textcolor{NavyBlue}{brush}, \textcolor{NavyBlue}{towel} & 7.7 & \textcolor{NavyBlue}{beam}, \textcolor{red}{oven}, \textcolor{NavyBlue}{mountain} \\ 
mountains, desert, sky& 0.0 & \textcolor{NavyBlue}{sky}, \textcolor{red}{building}, \textcolor{red}{wall} & 0.0 & \textcolor{NavyBlue}{brush}, \textcolor{NavyBlue}{sky}, \textcolor{red}{building} & 10.6 & \textcolor{NavyBlue}{mountain}, \textcolor{red}{fence}, \textcolor{NavyBlue}{backpack} \\ 
%outdoor-transport& 24.4 & \textcolor{NavyBlue}{road}, \textcolor{NavyBlue}{bridge}, \textcolor{NavyBlue}{sky} & 37.2 & \textcolor{red}{brush}, \textcolor{red}{sconce}, \textcolor{NavyBlue}{road} & 58.0 & \textcolor{NavyBlue}{fence}, \textcolor{red}{beam}, \textcolor{NavyBlue}{car} \\ 
%shopping-dining& 0.0 & \textcolor{NavyBlue}{vending machine}, \textcolor{NavyBlue}{newspaper}, \textcolor{red}{sky} & 16.8 & \textcolor{NavyBlue}{plate}, \textcolor{NavyBlue}{fluorescent}, \textcolor{NavyBlue}{brush} & 18.1 & \textcolor{NavyBlue}{beam}, \textcolor{red}{toilet tissue}, \textcolor{NavyBlue}{person} \\ 
%sports fields, parks& 0.0 & \textcolor{NavyBlue}{tree}, \textcolor{red}{floor}, \textcolor{red}{newspaper} & 8.7 & \textcolor{red}{fluorescent}, \textcolor{red}{brush}, \textcolor{NavyBlue}{sconce} & 30.4 & \textcolor{red}{swivel chair}, \textcolor{NavyBlue}{post}, \textcolor{NavyBlue}{fence} \\ 
water, ice, snow& 31.2 & \textcolor{red}{building}, \textcolor{red}{floor}, \textcolor{red}{road} & 68.4 & \textcolor{NavyBlue}{brush}, \textcolor{NavyBlue}{fluorescent}, \textcolor{red}{wall} & 85.3 & \textcolor{NavyBlue}{mountain}, \textcolor{red}{beam}, \textcolor{NavyBlue}{earth} \\ 
workplace& 64.3 & \textcolor{red}{sky}, \textcolor{NavyBlue}{floor}, \textcolor{NavyBlue}{wall} & 68.0 & \textcolor{NavyBlue}{fluorescent}, \textcolor{red}{sconce}, \textcolor{red}{brush} & 76.5 & \textcolor{NavyBlue}{swivel chair}, \textcolor{red}{post}, \textcolor{red}{beam} \\ 
 \toprule
\multicolumn{7}{l}{\textbf{least faithful}}\\
\toprule
\multirow{2}{*}{scene group} & \multicolumn{2}{c|}{most understandable} & \multicolumn{2}{c|}{somewhat understandable} & \multicolumn{2}{c}{least understandable} \\ \cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}
& TPR & concepts & TPR & concepts & TPR & concepts \\ \midrule 
comm-buildings & 79.3 & \textcolor{red}{seat}, \textcolor{red}{sink}, \textcolor{red}{plane} & 76.2 & \textcolor{NavyBlue}{building}, \textcolor{red}{grass}, \textcolor{NavyBlue}{house} & 73.1 & \textcolor{red}{floor}, \textcolor{red}{tree}, \textcolor{NavyBlue}{plant} \\ 
cultural-historical & 46.1 & \textcolor{red}{plane}, \textcolor{red}{case}, \textcolor{red}{bed} & 44.4 & \textcolor{NavyBlue}{building}, \textcolor{red}{road}, \textcolor{NavyBlue}{house} & 44.8 & \textcolor{NavyBlue}{sky}, \textcolor{NavyBlue}{wall}, \textcolor{NavyBlue}{chandelier} \\ 
home-hotel & 96.9 & \textcolor{red}{water}, \textcolor{red}{road}, \textcolor{red}{plane} & 92.3 & \textcolor{NavyBlue}{bed}, \textcolor{NavyBlue}{grass}, \textcolor{red}{field} & 91.4 & \textcolor{NavyBlue}{fireplace}, \textcolor{NavyBlue}{wall}, \textcolor{NavyBlue}{mirror} \\ 
indoor-cultural & 0.0 & \textcolor{red}{house}, \textcolor{red}{mountain}, \textcolor{red}{skyscraper} & 20.7 & \textcolor{NavyBlue}{house}, \textcolor{red}{tree}, \textcolor{red}{sea} & 41.3 & \textcolor{red}{mirror}, \textcolor{NavyBlue}{chandelier}, \textcolor{NavyBlue}{wall} \\  
mountains, desert, sky & 29.8 & \textcolor{red}{skyscraper}, \textcolor{red}{floor}, \textcolor{red}{sink} & 42.6 & \textcolor{NavyBlue}{mountain}, \textcolor{NavyBlue}{field}, \textcolor{red}{road} & 44.7 & \textcolor{red}{wall}, \textcolor{NavyBlue}{hill}, \textcolor{red}{house} \\ 
water, ice, snow & 58.0 & \textcolor{red}{case}, \textcolor{red}{skyscraper}, \textcolor{red}{sink} & 92.2 & \textcolor{red}{field}, \textcolor{NavyBlue}{water}, \textcolor{NavyBlue}{sea} & 78.4 & \textcolor{red}{wall}, \textcolor{red}{fireplace}, \textcolor{NavyBlue}{floor} \\ 
workplace & 22.0 & \textcolor{red}{house}, \textcolor{red}{water}, \textcolor{red}{mountain} & 74.1 & \textcolor{NavyBlue}{floor}, \textcolor{red}{cushion}, \textcolor{red}{sea} & 63.9 & \textcolor{NavyBlue}{floor}, \textcolor{red}{fireplace}, \textcolor{NavyBlue}{console table} \\ 
 \bottomrule
\end{tabular}
